HeadCraft: Modeling High-Detail Shape Variations for Animated 3DMMs

Current advances in human head modeling allow the generation of plausible-looking 3D head models via neural representations, such as NeRFs and SDFs. Nevertheless, constructing complete high-fidelity head models with explicitly controlled animation remains an issue. Furthermore, completing the head geometry based on a partial observation, e.g., coming from a depth sensor, while preserving a high level of detail is often problematic for the existing methods. We introduce a generative model for detailed 3D head meshes on top of an articulated 3DMM, simultaneously allowing explicit animation and high-detail preservation. Our method is trained in two stages. First, we register a parametric head model with vertex displacements to each mesh of the recently introduced NPHM dataset of accurate 3D head scans. The estimated displacements are baked into a hand-crafted UV layout. Second, we train a StyleGAN model to generalize over the UV maps of displacements, which we later refer to as HeadCraft. The decomposition of the parametric model and high-quality vertex displacements allows us to animate the model and modify the regions semantically. We demonstrate the results of unconditional sampling, fitting to a scan and editing. The project page is available at https://seva100.github.io/headcraft.

==> supp_fig_tex/fitting_w_and_noise_compn.tex <==
% \vspace{-0.2cm}
\begin{table}[t!]
    \centering
    \setlength{\tabcolsep}{0pt}
    \begin{tabular}{ccccc}
    $\mathcal{W}+$ & $\mathcal{W}+$ \& Noise & \hspace{0.3cm} & $\mathcal{W}+$ & $\mathcal{W}+$ \& Noise \\
    \includegraphics[width=0.11\textwidth,trim={4cm 1cm 0.5cm 1cm},clip]{} 
    & \includegraphics[width=0.11\textwidth,trim={4cm 1cm 0.5cm 1cm},clip]{}         
    & \hspace{0.4cm}
    & \includegraphics[width=0.11\textwidth,trim={4cm 1cm 0.5cm 1cm},clip]{}  
    & \includegraphics[width=0.11\textwidth,trim={4cm 1cm 0.5cm 1cm},clip]{} 
    \\
    \includegraphics[width=0.11\textwidth,trim={4cm 1cm 0.5cm 1cm},clip]{} 
    & \includegraphics[width=0.11\textwidth,trim={4cm 1cm 0.5cm 1cm},clip]{}         
    &  \hspace{0.4cm}
    & \includegraphics[width=0.11\textwidth,trim={4cm 1cm 0.5cm 1cm},clip]{}  
    & \includegraphics[width=0.11\textwidth,trim={4cm 1cm 0.5cm 1cm},clip]{} 
    \end{tabular}
    \captionof{figure}{
    The result of fitting the $w \in \mathcal{W}+$ latent code and subsequently the StyleGAN noise to a registered complete UV map.
    }
    \label{fig:fitting_w_and_noise_compn}
    \vspace{-0.4cm}
\end{table}

==> supp_fig_tex/seam.tex <==
\begin{table}[h!]
    \centering
    \setlength{\tabcolsep}{0pt}
    \begin{tabular}{cp{0.3cm}c}
    Standard UV & \hspace{0.3cm} & Custom UV \\
    \includegraphics[width=0.4\linewidth,trim={1cm 1cm 0.5cm 1cm},clip]{supp_fig/seam/standard_seam.jpg} 
    & \hspace{0.3cm}
    & \includegraphics[width=0.4\linewidth,trim={1cm 1cm 0.5cm 0cm},clip]{supp_fig/seam/new_seam.jpg} \\
    \end{tabular}
    \vspace{-0.2cm}
    \captionof{figure}{
    Demonstration of the custom UV seam annotation.
    %
    \textit{Standard UV} corresponds to the UV space shipped with the FLAME model.
    %
    \textit{Custom UV} stands for the handcrafted layout employed in our pipeline.
    %
    This layout simplifies learning sophisticated shape variations such as long hair in a consistent way.
    }
    \label{fig:seam}
\end{table}
